A Formalism and an Algorithm for Computing Pragmatic Inferences and Detecting Infelicities

Since Austin introduced the term ``infelicity'', the linguistic literature has been flooded with its use, but no formal or computational explanation has been given for it. This thesis provides one for those infelicities that occur when a pragmatic inference is cancelled. Our contribution assumes the existence of a finer grained taxonomy with respect to pragmatic inferences. It is shown that if one wants to account for the natural language expressiveness, one should distinguish between pragmatic inferences that are felicitous to defeat and pragmatic inferences that are infelicitously defeasible. Thus, it is shown that one should consider at least three types of information: indefeasible, felicitously defeasible, and infelicitously defeasible. The cancellation of the last of these determines the pragmatic infelicities. A new formalism has been devised to accommodate the three levels of information, called ``stratified logic''. Within it, we are able to express formally notions such as ``utterance U presupposes P'' or ``utterance U is infelicitous''. Special attention is paid to the implications that our work has in solving some well-known existential philosophical puzzles. The formalism yields an algorithm for computing interpretations for utterances, for determining their associated presuppositions, and for signalling infelicitous utterances that has been implemented in Common Lisp. The algorithm applies equally to simple and complex utterances and sequences of utterances.

==> introduction.tex <==
%auto-ignore

\chapter{Introduction}

Much of the research done in linguistic pragmatics makes extensive use
of the term {\em infelicity}. However, it seems that no approach
offers a formal or computational definition for this phenomenon. It is
the goal of this thesis to provide one. Unfortunately, the scope of
the phenomenon of infelicity is extremely large and not well-defined.
Apparently, the word was introduced by Austin~\shortcite{austin62} to
characterize performative utterances that fail.  But since then, it
has become fashionable to characterize anything that goes wrong as
infelicitous.  If a sentence is not syntactically or semantically
well-formed it is often said to be infelicitous; if an utterance is
not pragmatically well-formed it is said to be infelicitous too.  This
thesis is about pragmatic infelicities: those that occur when some
Gricean inferences are cancelled.

Chapter 2 is dedicated to a study of the relevant work in implicature
and presupposition from a perspective concerned primarily with aspects
of felicity. It is shown that besides the classical dichotomy of
pragmatic inferences in implicatures and presuppositions one should
take into consideration a dichotomy between felicitous defeasible and
infelicitous defeasible inferences. It is shown that the second
classification does not overlap the first one.

In order to capture pragmatic infelicities, we introduce a new
formalism called stratified logic. Chapter 3 contains the informal
intuitions that lie behind this new mathematical tool, and a
characterization of its syntax and semantics for the propositional and
first-order case.

Chapter 4 sheds some light on a fundamental difference between the
notions of lexical semantics and lexical pragmatics. It is shown that
an appropriate semantic and pragmatic characterization of the lexical
items and syntactical constructs in terms of stratified logic not only
provides a formal characterization for pragmatic infelicities but also
an adequate explanation for cancellations that implicatures and
presuppositions are subject to. Chapter 5 extends this work and shows
how the solution developed for simple utterances is appropriate
without any modifications for handling complex utterances. Thus, we
obtain a formalism and a computational method that signal infelicitous
utterances and determine their associated presuppositions independent
of their complexity. Our method works even for sequence of utterances,
a case that is omitted by previous research in the area.

The existential presuppositions carried by definite references are one
of the most problematic linguistic and philosophical issues. Chapter 7
is dedicated to a review of the work done in this area. It is shown
that most of the philosophical approaches are more concerned in
dealing with nonexistence and they fail to capture the existential
presuppositions, while most of the linguistic approaches are incapable
to accommodate nonexistent entities. We use a rich ontology \`{a} la
Hirst and a set of methodological principles that embed the essence of
Meinong's philosophy and Grice's conversational principles into a
stratified logic, under an unrestricted interpretation of the
quantifiers. The result is a logical formalism that yields a tractable
computational method that uniformly calculates all the presuppositions
of a given utterance, including the existential ones. A comparison
with Parsons's, Russell's, and Hobbs's work emphasizes the superiority
of our approach.

Chapter 8 is concerned with some implementation issues. Two annexes
are provided: one that contains the Lisp code of our implementation,
and one that contains the results computed by our program on a
representative set of examples.
